Interactive Modelling of Volumetric Musculoskeletal Anatomy

We present a new approach for modelling musculoskeletal anatomy. Unlike previous methods, we do not model individual muscle shapes as geometric primitives (polygonal meshes, NURBS etc.). Instead, we adopt a volumetric segmentation approach where every point in our volume is assigned to a muscle, fat, or bone tissue. We provide an interactive modelling tool where the user controls the segmentation via muscle curves and we visualize the muscle shapes using volumetric rendering. Muscle curves enable intuitive yet powerful control over the muscle shapes. This representation allows us to automatically handle intersections between different tissues (musclemuscle, muscle-bone, and muscle-skin) during the modelling and automates computation of muscle fiber fields. We further introduce a novel algorithm for converting the volumetric muscle representation into tetrahedral or surface geometry for use in downstream tasks. Additionally, we introduce an interactive skeleton authoring tool that allows the users to create skeletal anatomy starting from only a skin mesh using a library of bone parts.

==> todo.tex <==
\section{Color scheme}
You can import Illustrator color scheme from here - \url{https://color.adobe.com/search?q=RinatMuscle}
\section{To do}
% \hfill \break
% - Show tesselation
% \hfill \break
% - Compare to artist created muscles!
\hfill \break
add vector field on top of figures
\hfill \break
- Create builds for user study - \textbf{done}.
\hfill \break
- Need to find people for the user study - \textbf(Richard, Josh, Sarah, Jason(maybe)). \textbf{done}
% \hfill \break
% - Show how we can create different types of muscles, combining curves

\hfill \break
- More examples 
\hfill \break 
- Simulation \textbf{done with vismays code}
% \hfill \break 
% 1) Send Dave hand with muscles and fiber fields
% \hfill \break 
% 2) EMU framework simulation
% Options:  
% 1) (Complementary dynamics) Fully cartoony muscles - Rigid Bones drive the simulation. (set bones as boundary condition and the rest is driven by FEM, treat muscles as an "elastic" material that obeys the laws of physics)
% 2) (3rd) simulate the whole tet mesh but set different material parameters per tet (we know which tets are muscles and which tets fat/air/bones).
% 3) (VFX) Solve for muscle activation given the bone positions.
% 4) EMU framework - Muscles drive bones
\hfill \break 
Video:
Show interactive process at the start (Lion?)
Show fully rendered results (turn table animation?)
Show simulation

 
